Why is Differential Evolution Better than Grid Search for Tuning Defect Predictors?

Context: One of the black arts of data mining is learning the magic parameters which control the learners. In software analytics, at least for defect prediction, several methods, like grid search and differential evolution (DE), have been proposed to learn these parameters, which has been proved to be able to improve the performance scores of learners. Objective: We want to evaluate which method can find better parameters in terms of performance score and runtime cost. Methods: This paper compares grid search to differential evolution, which is an evolutionary algorithm that makes extensive use of stochastic jumps around the search space. Results: We find that the seemingly complete approach of grid search does no better, and sometimes worse, than the stochastic search. When repeated 20 times to check for conclusion validity, DE was over 210 times faster than grid search to tune Random Forests on 17 testing data sets with F-Measure Conclusions: These results are puzzling: why does a quick partial search be just as effective as a much slower, and much more, extensive search? To answer that question, we turned to the theoretical optimization literature. Bergstra and Bengio conjecture that grid search is not more effective than more randomized searchers if the underlying search space is inherently low dimensional. This is significant since recent results show that defect prediction exhibits very low intrinsic dimensionality-- an observation that explains why a fast method like DE may work as well as a seemingly more thorough grid search. This suggests, as a future research direction, that it might be possible to peek at data sets before doing any optimization in order to match the optimization algorithm to the problem at hand.

==> reply_to_reviewers.tex <==
\section*{Reply to Reviewers}

Thank you for your careful reviews. 

The main objection to this paper comes from Reviewer2 who argues that this is not a journal-level contribution.
As Reviewer2 correctly points in tuning is mentioned in many ML textbooks.  That said, our comment here is
that there is a  huge  gap between such statements and current practice.  In our view, the computational cost of tuning is the major factor
blocking researchers in applying this important technique. The value of this paper is to show that a widely-used tuning method (grid search-- which is very slow)
can be discarded in favor of a much faster method.

Now Reviewer2 was completely correct in noting that the prior draft did not motivate the need for truning.
What was {\bf missing} in that prior draft were notes on our literature reviews on the appalling state of SE analytics the lack of tuning across much of the research in that field. What that literature review showed was tuning is very rarely done. 

In any case, this paper now includes notes on that survey (see section 2.3) and the following figure:

\setcounter{figure}{0}
\begin{figure}[!h]
    \centering
    \includegraphics[width=3.5in]{pic/literature.pdf}
    \caption{Literature review about parameter tuning on 52 top cited defect prediction papers}

\end{figure}


As to other changes, we have made many changes based on your comments, detailed below. In summary, the major changes are:
\bi
\item Added two more evaluation measures AUC(pf, pd), AUC(20\%effort, pd) as requested.
\item Added a  paragraph in background about tuning literature review in defect prediction, which shows that how tuning was poorly explored in  defect prediction literature.
\item Added all grid search performance scores into the charts.
\item Added ``threats to validity'' section.
\item Fixed all issues related to charts: legends, labels, x-axis, y-axis.
\item Fixed all typos pointed out by reviewers.
\ei


\noindent{\textbf{ Reviewer 1}}

{\em This study assesses Grid search, random search and Differential Evolution algorithm for its effectiveness in tuning the parameters of two machine learning algorithms (CART and Random Forests) in order to construct efficient defect predictors. The methods for tuning parameters were assessed on 17 data sets using performance evaluation functions (G-mean and F-measure) and the cost (run-time). The authors have conducted an interesting study where they have discussed the reasons for the trends of the results. However, the following major revisions should be incorporated before the manuscript can be accepted for publication. 

The manuscript needs a lot of English corrections and proper reference numbers. These issues should be carefully addressed by the authors.}

We have carefully proofread the revised paper and have fixed   those incorrect reference numbers. 

{\em R1-1: The authors have optimized two performance metrics for defect predictors i.e. ``precision'' and ``F-measure''. It would be interesting to know whether the results would be same if the author's optimize, ``Balance'', ``Area Under the Receiver Operating Characteristic Curve'' and ``G-Mean''?}

Thank you for that comment. This paper uses more evaluation measures (not baseline of “G”-- even though we introduced those to defect prediction back in 2007-- since these are not widely used. What we did do is add the more standard measures of  AUC(pf, recall)   and AUC(effort=20\%,recall)
(Aside: why  AUC(effort=20\%,recall)? Please see \url{http://tiny.cc/auc20})

{\em R1-2: Figure 1 is incomplete. The authors have not added definition of several metrics like dit, npm, noc etc…}

Our apologies. We fixed that.

{\em R1-3: Page 3: ``we note that the general trend in SE data science papers is to explore defect prediction without tuning the parameters''. How can you report a general trend by stating only one example? The paper cited is not a review or survey.}

In a prior (and recent) paper, we offered such a review (*). We did not repeat that material in the first draft of this paper, which was our mistake. In this draft, we offer a summary of that material in Section 2.3 with updated information, which includes two latest paper about parameter tuning for defect prediction.

(*) W. Fu, T. Menzies, X. Shen, Tuning for software analytics: Is it really necessary?, Information and Software Technology 76 (2016) 135–146

{\em R1-4: Figure 4: What does the y-axis in the graph represent? The whole figure should be renamed into four parts a), b) c) and d)? what are the differences or similarities between the four figures? Why only statistically significant grid search results are shown? Where are the other grid search results?}

Thank you for that comment. We have fixed these as  you requested.

{\em R1-5: Section 3.2: Are the data sets balanced with almost equal number of defective and not defective classes? Are they imbalanced? If yes, what is the imbalance ratio? Would the imbalance ratio produce any change in results? Why or why not? Is this a possible validity threat to the study?}

With your permission, we’d rather not say anything on this point. We just completed a very extensive analysis of SMOTE which will submit to ESEM’17  (see a draft at \url{http://tiny.cc/imbalance}). So we have much to say on this point but it takes us into the interesting lang of unpublished results.  

{\em R1-6: Section 3.2.3: The authors have stated that the data is available in PROMISE repository but it is necessary to mention the release numbers of the selected data sets so that the study can be easily replicated.}

We endorse the reviewer's call to make all data sets in empirical SE papers available for long term access via some release number scheme.
Prompted by your suggestion, all the data is now available, with a persistent digital object identifier, at \url{http://tiny.cc/zd_data}.
For the information of the reviewer, we note that the DOI for that data set is 10.5281/zenodo.344970. We also note that readers of this article
can access that DOI as part of Reference~\cite{fu_wei_2017_344970}.

{\em R1-7: Result 1: ``DE is better than random search in a couple of data sets.''  what do you mean by a couple of data sets. It is a very vague term. What percentage of data sets? Or how many data sets?} 

We replace ``couple'' with ``majority'' which is a term with a much clearer meaning (i.e. more than half).

{\em R1-8: Figure 5: In this figure, ``lef'' and ``right'' is mentioned but there is no left and right. Again the figure should be broken into two parts and clearly mentioned. Also label the X-axis and Y-axis.}

Apologies! We fixed that.

{\em R1-9: Though, the authors have discussed in detail the external validity of the paper, a Threats to Validity: section is missing which should report the conclusion, construct, internal and external validity threats of the study.}

Apologies! We fixed that.


\noindent\textbf{ Minor Comments}

Thanks, we fixed all the following.
\bi
\item {\em R1-10: Abstract: ``We want to evaluate which method that can find''  ``We want to evaluate which method can find''}
\item {\em R1-11: Abstract: ``hours vs 54 days for grid search when both tuning Random Forest''. The meaning is not clear.}
\item {\em R1-12: Abstract: ``when both tuning Random Forest''. The meaning is not clear.}
\item {\em R1-13: Page 1: ``B oth paper''  ``Both paper''}
\item {\em R1-14: Page 2: ``Any method that focuses on parts of the code can miss defects in other areas so some sampling policy should be used to explore the rest of the system.'' Did you mean specific parts? }
\item {\em R1-15: Page 2: ``yet no more effective, than differential''  ``yet it is not more effective, than differential''}
\item {\em R1-16: Page 3, Section 2.1: ``There are increasing number of work''  ``There is an increasing number of wor''}
\item {\em R1-17: Page 3: on leaf notes ??? I think you mean leaf nodes.}
\item {\em R1-18: Page 3: Is it topic modeling? Or topic modelling?}
\item {\em R1-19: What is the full form of MLPs? What is CART? What is SE? What is LDA? The authors should define all acronym names at the first instance.}
\item {\em R1-20: Page 3, Section 2.2: ``various heuristics to reduce their search space''  ``various heuristics in order to reduce their search space''}
\item {\em R1-21: Page 3, Section 2.2: ``split on on''  ``split on''}
\item {\em R1-22: Page 3: ``This was another grid search paper that explored a range of tunings parameters, divided into 5 bins.'' What was divided into 5 bins?}
\item {\em R1-23: Page 3: ``Yet for tuning defect predictors, both groups reported the same results:''  ``Yet for tuning defect predictors, both groups reported the same results which are stated as follows:''}
\item {\em R1-24: Page 4, Section 2.3, last para: There are no proper citations in the para to specific reference numbers. Apart from this para, at several other places proper reference numbers are not mentioned. The authors are requested to go through the manuscript correctly to remove these errors.}
\item {\em R1-25: In page 4, the authors state ``Tuning offers a median improvement of 5\% to 15\%'' and ``For a third of data sets exploration, tuning can result in performance improvements of 30\% to 50\%''. What type of performance? Are the authors talking about classification performance? Were the improvement trends same for all performance metrics like AUC, precision etc. Please be specific. The median value of which performance metric improved???}
\item {\em R1-26: Page 4: As to automating grid search, it is simple to implement and parallelization is trivial;}
\item {\em R1-27: Page 5: ``Other parameters grid will generate in the same way.  will be generated in the same way'' OR ``are generated in the same way''}
\item {\em R1-28: Page 5: ``CART or Random Forests applied to release i+2''  ``CART or Random Forests and applied them to release i+2''}
\item {\em R1-29: Page 5: ``i and i+1 then tested on release i+2.''  ``i and i+1, and then tested on release i+2.''}
\item {\em R1-30: Page 5: ``According to Bergstra and Bengio [25], grid search (on a compute cluster)''  compute cluster or computer cluster?}
\item {\em R1-31: Page 5: ``That study ranked CART worst and Random Forests as best.''  ``That study ranked CART as the worst leaning technique and Random Forests as the best learning technique.''}
\item {\em R1-32: Page 5: ``In a demonstration of the impact of tuning, Fu et al. showed that they could''  ``However, in a demonstration of the impact of tuning, Fu et al. [reference no. missing]….''. The reference numbers are missing at a number of places.}
\item {\em R1-33: Page 5: ``Other parameters grid will generate in the same way.''  ``Other parameters grid will be generated in the same way.''}
\item {\em R1-34: Page 6: ``For example, when we tune for recall, we can achieve near 100\% recall but the cost of a near 100\% false alarms. Similarly, when we tune to minimize false alarms, we can achieve near 0\% false alarms but the cost of a near 0\% recall.''  ``For example, when we tune for recall, we can achieve near 100\% recall but 'at' the cost of a near 100\% false alarms. Similarly, when we tune to minimize false alarms, we can achieve near 0\% false alarms but 'at' the cost of a near 0\% recall.''}
\item {\em R1-35: Page 6: ``Acura \& Briand''  ``Arcuri and Briand''}
\item {\em R1-36: Page 6: ``Does tuning improve learners performance?''  ``Does tuning help in improving learner's performance?''}
\item {\em R1-37: Page 6: ``andF-Measure''  Space required.}
\item {\em R1-38: Page 6: ``what happens we run a learner using the default parameter'' ``what happens when we run a learner using the default parameter''}
\item {\em R1-39: Page 7: ``yellow triangle show''  ``yellow triangles show''}
\item {\em R1-40: Page 7: ``The similar pattern can be found when F is set as our tuning objective.''  ``A similar pattern is found when F-measure is used as our tuning objective.''}
\item {\em R1-41: Page 7: ``Note all the results where the red dots and blue squares are higher than green, particular in the results where we are tuning for precision.''  ``Note all the results where the red dots and blue squares are higher than green, particularly in the results where we are tuning for precision.''}
\item {\em R1-42: Page 8: ``just waste a lot of time to explore unnecessary space''  ``just wastes a lot of time to explore unnecessary spaces''}
\item {\em R1-43: Page 8: ``How might we assess the external validity''  ``How can we assess the external validity''}
\item {\em R1-44: Page 10: ``Further the tunings found in this way work as well, or better, than those found via grid search.'' : ``Further the tunings found in this way work is as good, or better, than those found via grid search.''}
\item {\em R1-45: Page 10:``often in holds in real data''  ``often it holds in real data''}
\ei 
All the above issues need to be carefully addressed by the authors. Therefore, the paper can only be accepted after these major revisions.



\noindent\textbf{Reviewer 2}

{\em This manuscript addresses the issue of hyper-parameter optimization for machine learning based defect predictors (CART and Random Forest) on static code attributes and compares grid search vs. differential evolution (vs. random search). Authors report that differential evolution is faster and at least as effective as grid search in parameter tuning for defect prediction. They conclude that the reason for this is the intrinsic low dimensionality of defect prediction data based on the premise that grid search is not more effective than heuristic search in case of low dimensional search space.

Pros:
\begin{itemize}
\item[+]
Empirical evaluation and comparison of two techniques for parameter optimization
\item[+]
Parameter optimization is a must in any artificial learning setting including defect prediction
\end{itemize}

Cons:
\begin{itemize}
\item[-]
Limited contribution
\item[-]
Wrong positioning in terms of research methodology 
\item[-]
No report on statistical test assumptions 
\item[-]
Problems with paper structure and research questions 
\item[-]
Main premise of the manuscript is built upon a logically flawed assumption
\end{itemize}

Detailed comments and suggestions for improvement:

R2-1: Limited Contribution: My main concern about this manuscript is its contribution to the body of knowledge. I can only acknowledge the comparison of two techniques as a contribution (caveat: only because it is the first comparison in defect prediction domain, they have been obviously studied in depth in other disciplines, e.g. ML). Authors list many contributions in the introduction, however, they are indeed quite trivial facts and machine learning textbook material that:}

Please see our comments at the start of this reply-to-reviewer section.

Please also accept our apologies for sending you a prior draft that did \underline{{\bf not}} include the core motivation for this work. Without that information,
we completely understand why you were negative on the previous draft.

{\em R2-2: fail to see a journal article level contribution considering the high quality level of IST journal. }

As we say above,
missing in the previous draft was the literature review that shows that most researchers do grid search.  As the literature review shown in the section 2.3, 80\% of 50 top cited defect prediction paper did not mention parameter tuning at all and they just used the default parameter for their learners. Only 4 paper
actually did parameter tuning and of those, three use grid search and the other one is our previous work with DE. 

We also wish to add that even though many textbooks mention the tuning problem, the support for funding effective tunings
is somewhat limited. For example:
\bi
\item
Consider the scikit-learn toolkit (data mining tool in python)~\footnote{http://tiny.cc/scikitlearn}.
That tool only offers grid search[1] is provided for parameter tuning. 
\item
The same is true for the ``R'' data mining
toolkit (see its {\em caret}~\footnote{http://tiny.cc/caret} package, which is a grid search algorthm. ). 
\item
Further, in the "WEKA" data mining toolkit~\footnote{http://tiny.cc/weka1}, grid search is the  built-in methods for parameter tuning.
\ei
Therefore, it is possible that the slow grid search is still a popular parameter tuning technique for data analytics practitioners. 
The point of our paper is
to document, very thoroughly, just how poorly data mining toolkit provider support grid search.
 


{\em R2-3: Research Methodology: I can relate with the authors that positioning the research method for MSR type research has been problematic in our community. As a matter of fact, most MSR research falls under the category of 'observational studies' and (unfortunately) wrongly posed as case studies/ experiments. However, in this case, the setup explained in the manuscript is a classic 'machine learning experiment', though argued as a case study rather than an experiment. (\url{http://tiny.cc/g3vpjy}). Specifically, this is a one factor (parameter optimization technique) with two levels (grid-search vs. differential evolution) controlled experiment, since all factors and conditions are fixed except for the one intervened by the authors. The observed effect (in performance of defect predictors) can be causally linked to the levels of the investigated factor. Establishing causal links is not possible in a case study. In
short, I'd recommend to reconsider the research method description, where the argumentation, e.g. by Cruzes et al., has nothing to do with the context of the paper for justifying the methodology.} 

We agree that our ``case study'' reference was just wrong. We also agree that your description of the methodology is correct, and actually obvious
from the rest of the text. Hence, we have deleted the section claiming this is a ``case study'' paper.

 

{\em R2-4: Statistical Tests: The manuscript reports no checks for the assumptions of statistical tests. To the best of my knowledge Scott-Knot is a ANOVA family test and requires certain assumptions, e.g. normality, to hold.  For the results to be valid, authors must ensure the reader that the choice of statistical test is proper based on the purpose and data at hand, rather than arguing the popularity of the specific test. }

Respectfully, we disagree. When Scott-Knot is originally proposed in the SE literature, it   usef Anova as the hypothesis test sub-routine (see \url{http://tiny.cc/sk}). In our work, we often have skewed distributions so we prefer non-parametric methods.
Hence, as described in Seciton 3.7 , we use a non-parametric statistical (bootstrapping)
and a nonparametric effect size test (A12).  

{\em R2-5: Structure and Research Questions: It is a bit weird to see the specific research questions only when reaching the 'Results' section. Research questions should be stated in the study design part and results should be reserved, well, for results.}

We fixed that.

{\em R2-6: As for the results section itself, I appreciate the authors efforts to highlight their findings in bulleted lists. However, result section is completely made up of bullets and they look like items from presentations slides. Please limit the use of bullets for the most important findings/ message and re=organize the content in textual form.}

We fixed that.


{\em R2-7: First research question is irrelevant by construct, e.g. 'Does tuning improve learners(') performance'. As I discussed in my criticism for alleged contributions, parameter tuning is a necessary step for all learning problems - no matter how immature SE community is in using ML methods.}


We agree that parameter tuning is a necessary step for all data mining problems. However, according to our literature review in defect prediction, 80\% of  52 highly cited paper did not acknowledge the impacts of parameter tuning at all(more details see R2-2) and only two papers about parameter tuning published in 2016 for tuning defect predictors. Therefore, in this paper, we need to stress the importance of parameter tuning as the first research question and allow more researchers in defect prediction field to notice this effect.

{\em R2-8: Third research question is also problematic for similar reasons. It simply does not make sense; grid search is an exhaustive search technique, whereas DE is an heuristic and by definition designed to avoid intractable nature of exhaustive methods, and to reach solutions faster at the risk of stopping at local optima.}

We quite take your point that, together, they do indeed address our main point , is DE most cost-effective than grid search for parameter tuning. However, for the sake of clear exposition, we ask the reviewer’s permission to offer them as different questions .

{\em R2-9: Problems with intrinsic low-dimensionality argument: Authors expect the reader to take a big leap of faith in taking their assumption for granted - and I cannot.  The argument of Bergstra and Bengio refers to the (intrinsic) dimensionality of the 'parameter search space' and NOT the original problem space (e.g. the dimensionality of defect data). These are two different domains. There is no logical/ empirical argument to link the low intrinsic dimensionality of the original problem space as a factor affecting the parameter optimization performance in the parameter search space.}

Respectfully, we disagree. Tree learners work by dividing the data space. Yet, they make many decisions during that process but please refer to table1 of \url{http://tiny.cc/2gwpjy}. Note how the classification accuracy of the results is very similar across each row. This means that despite all the different ways these learners explore the space (and each column reflects a different method) then the dominant controller of performance is the data space, not the decisions made by the learner on how that space is explored by the learner.

{\em R2-10: Parameter search space is determined by the learning algorithm, e.g. how many hyper parameters to tune, and it is independent of the underlying raw data on which the learner is 'mining'. Accordingly, the recommendation to choose the parameter tuning method based on the intrinsic dimensionality of 'data' is obsolete. Finally, for similar reasons, I do not see the relevance of the discussions of
Papakroni, and Provence, where both studies suggest simple models are enough because defect data is intrinsically low dimensional, and that's all. Indeed, one can question the validity of this if Papakroni have not tuned the parameters of their learners, e.g. parameter optimized leraners 'may' perform better than simple encoded cluster vectors.}

We actually disagree with you on this point. If tuning was ``independent of the underlying raw data on which the learner is mining''  then different data sets would have the same tunings. Yet they do not as shown by our previous results (see fig4 of https://arxiv.org/pdf/1609.01759.pdf).  Which means it is relevant to discuss Papakroni, and Provence.



{\em R2-11: Unfortunately, these are fundamental issues about the paper and require much more effort than a major revision to fix with a re-write. IMHO, comparison of two parameter optimization methods on defect data could make a good conference publication by itself if the manuscript is re-focused and pruned of its fundamental issues. }

Here again, we stress that in our opinion and based on our literature reviews, that parameter tuning is an open and urgent in SE analytics. Further, and this is what is exciting about our work, the effort required to conduct such tuning studies is far less than previously believed. We think that showing that a fast method (DE) works much better than a slower methods (grid search) is an important practical step forward top a batter generation of data analysis.

Other Issues:

{\em Figure 4: Please avoid colors and convert the figure to grey scale.   }

Since there are some overlaps between different tuning techniques for some measures, like AUC and F, 
it would be difficult to differentiate them without color even though we have different marks. 
So, with your permission, 
we prefer to keep the color as it better to read.  

 
